A non-abelian conjecture of Tate-Shafarevich type for hyperbolic curves

We state a conjectural criterion for identifying global integral points on a hyperbolic curve over $\mathbb{Z}$ in terms of Selmer schemes inside non-abelian cohomology functors with coefficients in $\mathbb{Q}_p$-unipotent fundamental groups. For $\mathbb{P}^1\setminus \{0,1,\infty\}$ and the complement of the origin in semi-stable elliptic curves of rank 0, we compute the local image of global Selmer schemes, which then allows us to numerically confirm our conjecture in a wide range of cases.

==> preamble.tex <==
\usepackage[all]{xy}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{array, url}
\usepackage{stmaryrd}
\usepackage{mathtools}
\usepackage{wasysym}
\usepackage{tensor}
\usepackage{mathdots}
\usepackage{amsbsy}
\usepackage{tikz-cd}

\usepackage[T2A,T1]{fontenc}
\DeclareSymbolFont{cyrillic}{T2A}{cmr}{m}{n}
\DeclareMathSymbol{\Sha}{\mathalpha}{cyrillic}{216}

%\usepackage
%[notref, notcite]
%{showkeys}
%\renewcommand\showkeyslabelformat[1]{ \mbox{\normalfont\tiny
%\ttfamily
%#1}}

\usepackage{latexsym}
\usepackage{amsxtra}


%\usepackage[margin=1in]{geometry}

\setlength{\marginparwidth}{1.3in}
\let\oldmarginpar\marginpar
\renewcommand\marginpar[1]{\-\oldmarginpar[\raggedleft\footnotesize #1]%
{\raggedright\footnotesize #1}}

%Anton's \segment command and \iquation environment
\newcounter{firstnumber}[section]
\newcounter{secondnumber}[firstnumber]
\newcounter{thirdnumber}[secondnumber]
\newcounter{fourthnumber}[thirdnumber]
\newcounter{fifthnumber}[fourthnumber]
\newcounter{currentdepth}

\renewcommand{\thefirstnumber}{\arabic{section}.\arabic{firstnumber}}
\renewcommand{\thesecondnumber}{\thefirstnumber.\arabic{secondnumber}}
\renewcommand{\thethirdnumber}{\thesecondnumber.\arabic{thirdnumber}}
\renewcommand{\thefourthnumber}{\thethirdnumber.\arabic{fourthnumber}}
\renewcommand{\thefifthnumber}{\thefourthnumber.\arabic{fifthnumber}}

\newcommand{\segment}[2]{%
    \setcounter{currentdepth}{1}%
    \def\thesubsection{\thefirstnumber}%
    \refstepcounter{firstnumber}\label{#1}%
    \addtocounter{subsection}{-1}%
    \subsection{#2}}
\newcommand{\ssegment}[2]{%
    \setcounter{currentdepth}{2}%
    \def\thesubsection{\thesecondnumber}%
    \refstepcounter{secondnumber}\label{#1}%
    \addtocounter{subsection}{-1}%
    \subsection{#2}}
\newcommand{\sssegment}[2]{%
    \setcounter{currentdepth}{3}%
    \def\thesubsection{\thethirdnumber}%
    \refstepcounter{thirdnumber}\label{#1}%
    \addtocounter{subsection}{-1}%
    \subsection{#2}}
\newcommand{\ssssegment}[2]{%
    \setcounter{currentdepth}{4}%
    \def\thesubsection{\thefourthnumber}%
    \refstepcounter{fourthnumber}\label{#1}%
    \addtocounter{subsection}{-1}%
    \subsection{#2}}

\newenvironment{iquation}
 {%
  \ifnum\thecurrentdepth=1 \refstepcounter{secondnumber}\def\theequation{\thesecondnumber}
    \else
    \ifnum\thecurrentdepth=2 \refstepcounter{thirdnumber}\def\theequation{\thethirdnumber}
      \else
      \ifnum\thecurrentdepth=3 \refstepcounter{fourthnumber}\def\theequation{\thefourthnumber}
        \else
        \ifnum\thecurrentdepth=4 \refstepcounter{fifthnumber}\def\theequation{\thefifthnumber}
        \fi
      \fi
    \fi
  \fi
  \begin{equation}
 }
{
\end{equation}
}


%aaa
\newcommand{\mar}{\marginpar}

%bbb

\newcommand{\bs}{\backslash}

%sets
\newcommand{\set}[2]{\big\{ #1 \; \big| \; #2 \big\} }

%categories
\newcommand{\Rep}{\operatorname{\bf{Rep}}}
\newcommand{\Vect}{\operatorname{\bf{Vect}}}


%arrows
\newcommand{\from}{\leftarrow}
\newcommand{\xto}{\xrightarrow}
\newcommand{\xfrom}{\xleftarrow}
\newcommand{\surj}{\twoheadrightarrow}

%operations on modules, morphisms, filtrations
\newcommand{\Cok}{\operatorname{Cok}}
\newcommand{\gr}{\operatorname{gr}}
\newcommand{\sgn}{\operatorname{sgn}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\rec}{\operatorname{rec}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\Gal}{\operatorname{Gal}}



%object formation
\newcommand{\Spec}{\operatorname{Spec}}
\newcommand{\Spf}{\operatorname{Spf}}
\newcommand{\Spm}{\operatorname{Spm}}
\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Div}{\operatorname{Div}}
\newcommand{\Li}{\operatorname{Li}}
\newcommand{\Cone}{\operatorname{Cone}}

%homs, ends, exts
\newcommand{\fHom}{\operatorname{\mathbb{H}\mathrm{om}}}
\newcommand{\Hom}{\operatorname{Hom}}
%\newcommand{\hom}{\operatorname{hom}}
\newcommand{\Ext}{\operatorname{Ext}}
\newcommand{\Isom}{\operatorname{Isom}}
\newcommand{\End}[1]{\mathrm{End} \, {#1}}
\newcommand{\iEnd}{\mathscr{E}\hspace{-.2 ex}nd \,}
\newcommand{\fAut}{\operatorname{\mathbb{A}\mathrm{ut}}}
\newcommand{\Aut}{\mathrm{Aut}\,}
\newcommand{\fEnd}{\mathbb{E}\mathrm{nd}}

\newcommand{\Fil}{\operatorname{Fil}}
\newcommand{\ad}{\operatorname{ad}}
\newcommand{\Lie}{\operatorname{Lie}}

%ccc
\newcommand{\Mod}{\operatorname{Mod}}

%fonts
\newcommand{\m}[1]{\mathrm{#1}}
\newcommand{\fk}[1]{\mathfrak{#1}}
\newcommand{\s}[1]{\mathscr{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\cl}[1]{\mathcal{#1}}
\newcommand{\bld}[1]{\textbf{#1}}

%greek
\newcommand{\la}{\lambda}
\newcommand{\ka}{\kappa}
\newcommand{\si}{\sigma}
\newcommand{\ze}{\zeta}
\newcommand{\ga}{\gamma}
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}

%groups, fields, rings
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\Ga}{{\mathbb{G}_a}}
\newcommand{\Gm}{{\mathbb{G}_m}}
\newcommand{\Qp}{{\QQ_p}}
\newcommand{\Zp}{{\ZZ_p}}
\newcommand{\Fp}{{\FF_p}}
\newcommand{\Qbar}{{\overline{\QQ}}}

%single letters in special fonts
\newcommand{\V}{\bb{V}}
\newcommand{\ZZ}{\bb{Z}}
\newcommand{\CC}{\bb{C}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\nN}{\fk{n}}
\newcommand{\gG}{\fk{g}}
\newcommand{\NN}{\bb{N}}
\newcommand{\QQ}{\bb{Q}}
\newcommand{\RR}{\bb{R}}
\newcommand{\PP}{\bb{P}}
\newcommand{\UU}{\bb{U}}
\newcommand{\Uu}{\mathcal{U}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\Dd}{\mathcal{D}}
\newcommand{\Tt}{\mathcal{T}}
\newcommand{\FF}{\bb{F}}
\renewcommand{\AA}{\bb{A}}
\newcommand{\ssf}{\mathcal{O}}
\newcommand{\Oo}{\mathcal{O}}
\newcommand{\Gg}{\mathcal{G}}
\newcommand{\Kk}{\mathcal{K}}
\newcommand{\Hh}{\mathcal{H}}
\newcommand{\Aa}{\mathcal{A}}
\newcommand{\Xx}{\mathcal{X}}
\newcommand{\Yy}{\mathcal{Y}}
\newcommand{\SSS}{{\bf S}}
\newcommand{\aA}{\fk{a}}
\newcommand{\vV}{\fk{v}}
\newcommand{\Ee}{\mathcal{E}}
\newcommand{\Ll}{\mathcal{L}}


%decorations
\newcommand{\inv}{^{-1}}
\newcommand{\til}{\widetilde}

%Diagrams
\newcommand{\areq}{\ar@{=}}
\newcommand{\suphook}{\ar@{^(->}}
\newcommand{\subhook}{\ar@{_(->}}


%%% ddd from Stefan

\newcommand{\inj}{\hookrightarrow}
\newcommand{\To}{\;\longrightarrow\;}
\newcommand{\iso}{\stackrel{\sim}{\to}}
\newcommand{\liso}{\;\stackrel{\sim}{\longrightarrow}\;}
%\newcommand{\Mapsto}{\;\longmapsto\;}
%conflicts with stmaryrd package
\newcommand{\pfeil}[1]{\stackrel{#1}{\to}}
\newcommand{\lpfeil}[1]{\stackrel{#1}{\To}}
\newcommand{\gen}[1]{\mathopen\langle#1\mathclose\rangle}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\Bigl\lvert#1\Bigr\rvert}


%%%% eee Article specific commands
\newcommand{\Shah}{\operatorname{Shah}}
\newcommand{\loc}{\operatorname{loc}}

\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\newcommand{\rTo}{\to}

\newcommand{\Sel}{\operatorname{Sel}}

\newcommand{\Poneminusthreepoints}{\PP^1\setminus\{0,1,\infty\}}
\newcommand{\thrpl}{\PP^1 \setminus \{0,1,\infty\}}

\newcommand{\MTG}{\operatorname{\mathbf{MTG}}}
\newcommand{\MTLisse}{\operatorname{\mathbf{MTLisse}}}
\newcommand{\MTFphi}{\operatorname{\mathbf{MTF\varphi}}}
\newcommand{\mtEtQpf}{\operatorname{\tensor*[^{\m{mt}}]{\textrm{\'Et}}{^\Qp_f}}}
\newcommand{\mtdRQp}{\operatorname{\tensor*[^{\m{mt}}]{\dR}{}(\Qp)}}
\newcommand{\mtGQ}	{
						\operatorname	{
										\tensor*[^{\m{mt}}]{G}{^\QQ}
										}
						}
\newcommand{\mtMot}{\operatorname{\tensor*[^{\m{mt}}]{Mot}{^\QQ}}}
\newcommand{\mtMotZSinv}{\mtMot(\ZSinv)}
\newcommand{\Mot}{{\bf Mot}}
\newcommand{\Fphi}{\boldsymbol {F\phi} }

\newcommand{\udr}{U^{dR}}
\newcommand{\uet}{U^{\acute{e}t}}

\newcommand{\zpn}{\ze_{p^n}}
\newcommand{\Qzpn}{\QQ(\zpn)}

\newcommand{\HTn}{G_{T,n}}
\newcommand{\GTn}{G_{T,n}}
\newcommand{\KTn}{K_{T,n}}
\newcommand{\HTinfty}{G_{T,\infty}}
\newcommand{\GTinfty}{G_{T,\infty}}
\newcommand{\KTinfty}{K_{T,\infty}}

\newcommand{\Zpn}{{\ZZ/p^n}}
\newcommand{\Zpm}{{\ZZ/p^m}}
\newcommand{\Zpstar}{\ZZ_p^*}
\newcommand{\Zpnstar}{(\ZZ/p^n)^*}
\newcommand{\Fpstar}{\FF_p^*}

\newcommand{\mupn}{\mu_{p^n}}

\newcommand{\Ttilde}{{\widetilde{T}}}

\newcommand{\hh}{\fk{h}}

\newcommand{\tbp}{\vec{01}}

\newcommand{\dR}{{\rm {dR}}}
\newcommand{\dRp}{{\rm{dR}_p}}
\newcommand{\et}{{\textrm {\'et}}}
\newcommand{\mot}{{\rm {mot}}}

\newcommand{\pioneinfty}{\pi_1^{[\infty]}}
\newcommand{\pionetwo}{\pi_1^{[2]}}
\newcommand{\pione}[1]{\pi_1^{[#1]}}
\newcommand{\pioneinftyet}{\pi_{1,\textrm{\'et}}^{[\infty]}}
\newcommand{\pionetwoet}{\pi_{1,\textrm{\'et}}^{[2]}}
\newcommand{\pioneet}[1]{\pi_{1,\textrm{\'et}}^{[#1]}}
\newcommand{\pioneinftydRp}{\pi_{1,\textrm{dR}_p}^{[\infty]}}
\newcommand{\pionetwodRp}{\pi_{1,\textrm{dR}_p}^{[2]}}
\newcommand{\pionedRp}[1]{\pi_{1,\textrm{dR}_p}^{[#1]}}

\newcommand{\bKatwo}{ {_b\Kk}_a \langle 2 \rangle }
\newcommand{\bKaone}{ {_b\Kk}_a \langle 1 \rangle }
\newcommand{\starKaone}{ {_*\Kk}_a \langle 1 \rangle }
\newcommand{\ibstarbKaone}{ (i_{b*}) (\bKaone) }

\newcommand{\bKa}{{ {_bK}_a}}
\newcommand{\bPa}{{ {_bP}_a}}
\newcommand{\bYa}{{ {_bY}_a }}
\newcommand{\bXa}{{ {_bX}_a }}
\newcommand{\bAa}{{ {_bA}_a }}

\newcommand{\kabar}{\overline\ka}
\newcommand{\kabarm}{\kabar_m}
\newcommand{\kbt}{\kabarm(2)}

\newcommand{\ZSinv}{\ZZ[S\inv]}

\newcommand{\Sbar}{\overline S}
\newcommand{\SSSbar}{\overline \SSS}
\newcommand{\Untimesn}{U^{n \times n}}
\newcommand{\UntimesnFphi}{U^{n \times n, F\phi}}
\newcommand{\Un}{U^n}
\newcommand{\Unom}{U^{n, \om}}
\newcommand{\UnFphi}{U^{n,F\phi}}
\newcommand{\nn}{\nN^n}
\newcommand{\nntimesn}{\nN^{n \times n}}
\newcommand{\nnFphi}{\nN^{n, F\phi}}
\newcommand{\nntimesnFphi}{\nN^{n \times n, F\phi}}

\newcommand{\bS}{{\bf S}}
\newcommand{\bX}{\bar X}
\newcommand{\bF}{\bar F}
\newcommand{\pip}{\pi_{[2]}}
\newcommand{\Z}{\bb Z}
\newcommand{\cH}{\Hh}
\newcommand{\Q}{\QQ}
\newcommand{\cG}{\Gg}
\renewcommand{\t}{\tau}

\newcommand{\tbX}{\tilde \bX}
\newcommand{\ra}{\to}
\newcommand{\rOnto}{\surj}
\newcommand{\invlim}{\underset \from \lim}
\renewcommand{\O}{\Oo}
\newcommand{\cX}{\Xx}
\newcommand{\A}{\AA}
\newcommand{\z}{\zeta}
\renewcommand{\P}{\PP}
\newcommand{\cE}{\Ee}
\newcommand{\D}{\Delta}
\renewcommand{\a}{\al}
\renewcommand{\b}{\be}
\newcommand{\Exp}{\operatorname{Exp}}
\newcommand{\bE}{\bar E}
\newcommand{\piet}{\pi_1^\et(\bar X, b)}

\newcommand{\Fr}{\operatorname{Fr}}

\newcommand{\Id}{\operatorname{Id}}

%%remove allcaps or smallcaps from amsart title (author, section):
%\usepackage{etoolbox}
%\makeatletter
%\patchcmd{\@settitle}{\uppercasenonmath\@title}{}{}{}
%%\patchcmd{\@setauthors}{\MakeUppercase}{}{}{}
%%\patchcmd{\section}{\scshape}{}{}{}
%\makeatother

\raggedbottom

